OGB-LSC: A Large-Scale Challenge for Machine Learning on Graphs

Enabling effective and efficient machine learning (ML) over large-scale graph data (e.g., graphs with billions of edges) can have a great impact on both industrial and scientific applications. However, existing efforts to advance large-scale graph ML have been largely limited by the lack of a suitable public benchmark. Here we present OGB Large-Scale Challenge (OGB-LSC), a collection of three real-world datasets for facilitating the advancements in large-scale graph ML. The OGB-LSC datasets are orders of magnitude larger than existing ones, covering three core graph learning tasks -- link prediction, graph regression, and node classification. Furthermore, we provide dedicated baseline experiments, scaling up expressive graph ML models to the massive datasets. We show that expressive models significantly outperform simple scalable baselines, indicating an opportunity for dedicated efforts to further improve graph ML at scale. Moreover, OGB-LSC datasets were deployed at ACM KDD Cup 2021 and attracted more than 500 team registrations globally, during which significant performance improvements were made by a variety of innovative techniques. We summarize the common techniques used by the winning solutions and highlight the current best practices in large-scale graph ML. Finally, we describe how we have updated the datasets after the KDD Cup to further facilitate research advances. The OGB-LSC datasets, baseline code, and all the information about the KDD Cup are available at https://ogb.stanford.edu/docs/lsc/ .

==> issues.tex <==
% Although \nameshort{} has quickly spurred a surge of ML advances for moderate-scale graphs, the advances for large graphs with billions of edges or millions of graphs have still been limited.
Despite the emerging developments of graph ML for small- to medium-scale graphs (\eg, the traditional datasets---Cora and CiteSeer~\citep{yang2016revisiting}, and the recent \nameshort{} datasets, the advances for large graphs with billions of edges or millions of graphs have been extremely limited.
We attribute this to the lack of (1) suitable large-scale datasets and (2) dedicated scaling effort. We detail each of these points below.

\xhdr{Lack of suitable large-scale datasets}
Many classical graph datasets are extremely small in scale. Even for \nameshort{}, the majority of the datasets (14 out of 15) are up to either tens of millions of edges or half a million graphs.
The only large-scale dataset (with around a billion edges) available in \nameshort{} is on classical semi-supervised node classification over a homogeneous graph, \ie, \texttt{ogbn-papers100M}.
Although a good starting point, the task is rather simple and does not reflect the realistic challenges of large-scale graph tasks, namely, (1) handling the heterogeneity of graphs (\ie, a graph containing different node and edge types), and (2) performing large-scale link prediction. 
% Without suitable public datasets reflecting these challenges, it is hard for the community to work on the important challenges.
Below, we detail each challenge, highlighting its importance and research opportunities.

\yx{not sure about the point to argue about (2) link prediction and its associated paragraph? I might be lost, What is the purpose here}
\wh{That's a good point. We do not need to argue too much about link prediction. We just need to say there is no large-scale link/graph-level prediction datasets.}

First, heterogeneous graphs are prevalent in almost all kinds of large-scale graphs, \eg, social networks containing nodes for people, schools, companies, and places, as well as recommender systems containing nodes for users and items. However, many scalable graph methods based on feature/label propagation~\citep{wu2019simplifying,rossi2020sign,chen2020scalable,huang2020combining,bojchevski2020scaling} and mini-batch graph sampling~\citep{hamilton2017inductive,chen2018fastgcn,huang2018adaptive,zou2019layer,chiang2019cluster,zeng2019graphsaint} have been developed specifically for homogeneous graphs, and it remains largely an open question of how to adapt them effectively to large-scale heterogeneous graphs. 

Second, link prediction is also prevalent in large-graph applications, \eg, predicting new friendships in social networks, recommending items to users in recommender systems, and completing missing triplets in knowledge graphs.
Link prediction can be considered as node-level prediction, where the prediction domain spans the entire nodes in a graph. For a large graph, identifying the exact target node out of a huge number of candidate nodes requires extremely fine-grained prediction.
Moreover, link prediction typically involves learning unique embeddings for each node. 
Significant research is needed to efficiently learn the gigantic embedding matrix that can make highly fine-grained prediction.

\xhdr{Lack of dedicated scaling efforts}
Even on the rather simple \texttt{ogbn-papers100M} dataset, research effort has been limited to cheap propagation of node features/labels along graph structure ~\citep{wu2019simplifying,rossi2020sign,huang2020combining}. 
Although many advanced models and mini-batch training algorithms have been developed for medium-scale graphs~\citep{hamilton2017inductive,chen2018fastgcn,huang2018adaptive,zou2019layer,chiang2019cluster,zeng2019graphsaint}, there has been little dedicated research effort to scale them up and compare them on large-scale graphs, let alone develop new methods. 
We attribute this to the lack of common public datasets, scarcity of common codebase for ML on large-scale graph data, as well as the inherent difficulty in scaling up ML models to large data.
%\michele{why is that? lack of interest from researchers? hardware limitations? fundamental technical challenges? we need to elaborate.}

It is worth noting that in industry, many notable system-oriented efforts have emerged over the past few years to scale up graph ML models to large graphs. 
These include PinSAGE by Pinterest~\citep{ying2018graph}, AliGraph by Alibaba~\citep{zhu2019aligraph}, DGL by Amazon~\citep{wang2019dgl,zheng2020distdgl,zheng2020dgl}, Pytorch BigGraph by Facebook~\citep{lerer2019pytorch}, and PSGraph by Tencent~\citep{jiang2020psgraph}. Although promising, the datasets and implementation are often not made publicly available, and there is no standardized benchmark and evaluation protocol, making it hard for the community to keep track of the progress and to follow up. 
Moreover, these efforts have focused primarily on building fast and memory-efficient graph ML systems rather than comparing different methods and developing more advanced ones for large-scale graphs.
\challengeshort{} aims to build community-based dedicated research effort and standardized benchmark. We believe this would significantly facilitate the development of state-of-the-art models and their effective training algorithms.

\wh{I agree. I think we need to emphasize that "research" effort is lacking. Industry papers are more for system aspects, not algorithmic and modeling aspects.}
\michele{I think this paragraph above is EXTREMELY important, and having it at the end of Sec 2 is too late. Most of the reviewers form a very strong opinion about the paper after just reading the introduction, and if they are knowledgeable about graph ML, they will question why we are not talking at all about what already exists. Starting from the abstract, every time we mention that there's been a lack of scaling efforts, one can wonder "what about aligraph, pinsage, biggraph, etc.?" and start to think we don't really know what we are talking about.}

% We believe dedicated effort for large graphs would significantly advance the state-of-the-art for the following reasons.
% First, given a huge amount of data to learn from, more advanced expressive models would significantly outperform the simple baseline models based on cheap label/feature propagation.
% Moreover, effective mini-batching techniques become important, given that the number of nodes and edges that can be put in a single mini-batch is an extremely tiny fraction of the entire graph.
% Beyond advancing models and algorithms, their efficient implementation on specialized hardwares becomes crucial in handling large graphs, necessitating further effort in the intersection between software and hardware.


==> package.tex <==
\begin{wrapfigure}{r}{0.6\textwidth}
\vspace{-0.3cm}
\begin{lstlisting}[title={Code Snippet 1: \textbf{OGB Python package}},captionpos=b]
  ### Dataset object
  >>> from ogb.lsc import MAG240MDatase
  >>> dataset = MAG240MDataset()
  # Get split
  >>> dataset.get_idx_split(`train`)
  ### Evaluator object
  >>> from ogb.lsc import MAG240MEvaluator
  >>> evaluator = MAG240MEvaluator()
  # standardized evaluation
  >>> evaluator.eval(...)
  # saving the test prediction
  >>> evaluator.save_test_submission(...)
\end{lstlisting}
\vspace{-0.3cm}
\end{wrapfigure}
To make our datasets easily accessible, we have integrated them into the \nameshort{} Python package.\footnote{\url{https://github.com/snap-stanford/ogb}}
As shown in the Code Snippet 1, this allows our large datasets to be downloaded and processed with a few lines of code. 
In addition, for each dataset, we provide the evaluator object that evaluates and saves model's predictions (on the hidden test set) in a standardized way, making the test submission easy and reliable.
In our website,\footnote{\url{https://ogb.stanford.edu/kddcup2021/}} we provide the detailed tutorial of the package usage for each dataset.

